PNP: Fast Path Ensemble Method for Movie Design

How can we design a product or movie that will attract, for example, the interest of Pennsylvania adolescents or liberal newspaper critics? What should be the genre of that movie and who should be in the cast? In this work, we seek to identify how we can design new movies with features tailored to a specific user population. We formulate the movie design as an optimization problem over the inference of user-feature scores and selection of the features that maximize the number of attracted users. Our approach, PNP, is based on a heterogeneous, tripartite graph of users, movies and features (e.g., actors, directors, genres), where users rate movies and features contribute to movies. We learn the preferences by leveraging user similarities defined through different types of relations, and show that our method outperforms state-of-the-art approaches, including matrix factorization and other heterogeneous graph-based analysis. We evaluate PNP on publicly available real-world data and show that it is highly scalable and effectively provides movie designs oriented towards different groups of users, including men, women, and adolescents.

==> 020data.tex <==
The IMDB dataset consists of 1,893 movies with their features and ratings. The overview of the dataset is provided in Table~\ref{tab:IMDB}.

\begin{table}[htbp]
  \centering
  \caption{Features in the IMDB dataset.}
    \begin{tabular}{rr}
    \toprule
    \textbf{Features} & \multicolumn{1}{c}{\textbf{Counts}} \\
    \midrule
    \textbf{Total} & 58,918 \\
    \textbf{Movies} & 1,893 \\
    \textbf{Directors} & 947 \\
    \textbf{Producers} & 5,231 \\
    \textbf{Production Companies} & 1,209 \\
    \textbf{Actors} & 51,500 \\
    \textbf{Genre} & 27 \\
    \textbf{Seasons} & 4 \\
    \bottomrule
    \end{tabular}
  \label{tab:IMDB}
\end{table}




\subsection{Frequent Itemsets}

By using Ferenc Bodon's implementation for frequent item mining (apriori algorithm) with support $s=0.5\%$, we get several frequent $k$-itemsets ($k = 2, \ldots, 5$). Specifically, there are 516 frequent itemsets of size at least 2, which appear at least 10 times. Their distribution is given in Table~\ref{tab:frequentItemsets}. Table~\ref{tab:combosByType} shows which combinations of features appear most frequently together.

\begin{table}[htbp]
  \centering
  \caption{Frequent itemsets with support $s=0.5\%$.}
    \begin{tabular}{cr}
    \toprule
    \textbf{k} & \multicolumn{1}{c}{\textbf{\# itemsets}} \\
    \midrule
    1	  & 689 \\
    2     & 348 \\
    3     & 135 \\
    4     & 29 \\
    5     & 4 \\
    \bottomrule
    \end{tabular}
  \label{tab:frequentItemsets}
\end{table}

\textbf{Dependencies between features.} Our first goal is to see whether the features are dependent or independent. To this end, we focus on the frequent itemsets, and specifically sets of 2 items. If the items in the 2-itemsets are dependent, then the $k$-itemsets (for $k>1$) will be dependent as well. In this section, we use item and feature interchangeably. Let A be the event that feature 1 contributes to a movie, and B the event that feature 2 contributes to a movie. Then, to evaluate if A and B are independent we compute the probabilities $P(AB)$, $P(A)$, and $P(B)$, and check if $P(AB) = P(A) \cdot P(B)$. 

By following this procedure, we found that the 348 frequent pairs are all dependent. Therefore, there are dependencies between the supersets as well.

\begin{table}[htbp]
  \centering
  \caption{Types of features often occurring together.}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{rrrrr}
    \toprule
    \textbf{Count} & \textbf{Feature 1} & \textbf{Feature 2 } & \textbf{Feature 3} & \textbf{Feature 4} \\
    \midrule
    68    & genre & performer &       &  \\
    59    & genre & season &       &  \\
    46    & genre & genre & season &  \\
    38    & genre & producer &       &  \\
    36    & genre & genre &       &  \\
    31    & producer & productCompanies &       &  \\
    30    & producer & producer &       &  \\
    25    & genre & productCompanies &       &  \\
    19    & productCompanies & season &       &  \\
    16    & producer & season &       &  \\
    15    & producer & producer & productCompanies &  \\
    15    &       &       &       &  \\
    11    & genre & producer & producer &  \\
    11    & genre & genre & genre &  \\
    10    & producer & producer & producer &  \\
    5     & producer & producer & producer & productCompanies \\
    5     & performer & producer &       &  \\
    5     & genre & producer & productCompanies &  \\
    5     & genre & performer & producer &  \\
    5     & director & genre &       &  \\
    4     & producer & producer & season &  \\
    4     & performer & season &       &  \\
    4     & performer & productCompanies &       &  \\
    4     & performer & performer &       &  \\
    4     & genre & producer & producer & productCompanies \\
    4     & genre & producer & producer & producer \\
    4     & genre & genre & performer &  \\
    4     & director & genre & genre &  \\
    3     & genre & performer & productCompanies &  \\
    3     & genre & performer & performer &  \\
    2     & producer & producer & producer & producer \\
    2     & performer & producer & productCompanies &  \\
    2     & performer & producer & producer &  \\
    2     & genre & performer & producer & producer \\
    2     & genre & genre & productCompanies &  \\
    2     & genre & genre & genre & season \\
    2     & director & productCompanies &       &  \\
    2     & director & performer &       &  \\
    2     & director & genre & productCompanies &  \\
    2     & director & genre & performer & productCompanies \\
    2     & director & genre & performer &  \\
    \bottomrule
    \end{tabular}
    }
  \label{tab:combosByType}
\end{table}


\begin{table*}[ht!]
  \centering
  \caption{Lasso Regression}
  \resizebox{\textwidth}{!}{
\begin{tabular}{rrrrrrr}
    \toprule
          & \multicolumn{3}{c}{\textbf{Lasso Regression with 5-fold C.V.}} & \multicolumn{3}{c}{\textbf{Linear Regression  with 5-fold C.V.}} \\
    \midrule
    \multicolumn{1}{c}{\textbf{Features}} & \multicolumn{1}{c}{\textbf{min MSE}} & \multicolumn{1}{c}{\textbf{SE}} & \multicolumn{1}{c}{\textbf{lambda}} & \multicolumn{1}{c}{\textbf{min MSE}} & \multicolumn{1}{c}{\textbf{mean MSE}} & \multicolumn{1}{c}{\textbf{std MSE}} \\
    >= 2 occur. singletons & 1.0993 & 0.0152 & 0.04  & 20.9271 & 28.6743 & 8.5617 \\
    >= 10 occur. singletons & 1.0395 & 0.0533 & 0.0251 & 1.5448 & 1.5974 & 0.0467 \\
    >= 10 occur. single. + pairs & 1.0303 & 0.0328 & 0.0303 & 3.025 & 3.3704 & 0.3498 \\
    >= 10 occur. pairs & 1.1103 & 0.0327 & 0.0174 & 4.0232 & 16.3084 & 17.3369 \\
    >= 10 occur. single. + pairs + triplets & 1.0452 & 0.0526 & 0.0276 & 2.9254 & 3.9114 & 0.8767 \\
    \bottomrule
    \end{tabular}
    }
  \label{tab:lasso}
\end{table*}

\begin{table*}[ht!]
  \centering
  \caption{Lasso Regression}
  \resizebox{\textwidth}{!}{
\begin{tabular}{rcrrrrrrrrr}
    \toprule
          & \multicolumn{9}{c}{\textbf{Lasso Regression with 5-fold C.V.}}        & \textbf{Linear Regression } \\
          & \multicolumn{9}{c}{\textbf{}}        & \textbf{ with 5-fold C.V.} \\
    \midrule
    \multicolumn{1}{c}{\textbf{Features}} & \textbf{Number of} & \multicolumn{1}{c}{\textbf{non-zero}} & \multicolumn{1}{c}{\textbf{\% Sparsity}} & \multicolumn{1}{c}{\textbf{Coeff.}} & \multicolumn{1}{c}{\textbf{Coeff.}} & \multicolumn{1}{c}{\textbf{Coeff.}} & \multicolumn{1}{c}{\textbf{Top-30}} & \multicolumn{1}{c}{\textbf{Top-30}} & \multicolumn{1}{c}{\textbf{Top-30}} & \multicolumn{1}{c}{\textbf{non-zero}} \\
    \multicolumn{1}{c}{\textbf{}} & \textbf{features} & \multicolumn{1}{c}{\textbf{coeff.}} & \multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{Singletons}} & \multicolumn{1}{c}{\textbf{Pairs}} & \multicolumn{1}{c}{\textbf{Triplets}} & \multicolumn{1}{c}{\textbf{singletons}} & \multicolumn{1}{c}{\textbf{pairs}} & \multicolumn{1}{c}{\textbf{triplets}} & \multicolumn{1}{c}{\textbf{coeff}} \\
    >= 2 occur. singletons & 14028 & 408   & 97.09\% & 408   & N/A   & N/A   & 30    & N/A   & N/A   & 1437 \\
    >= 10 occur. singletons & 621   & 211   & 66.02\% & 211   & N/A   & N/A   & 30    & N/A   & N/A   & 620 \\
    >= 10 occur. single. + pairs & 969   & 207   & 78.64\% & 161   & 46    & N/A   & 23    & 7     & N/A   & 899 \\
    >= 10 occur. pairs & 348   & 141   & 59.48\% & N/A   & 141   & N/A   & N/A   & 30    & N/A   & 100 \\
    >= 10 occur. single. + pairs + triplets & 1104  & 235   & 78.71\% & 179   & 45    & 11    & 20    & 7     & 3     & 951 \\
    \bottomrule
    \end{tabular}
    }
  \label{tab:lassoCoeff}
\end{table*}

\subsection{Lasso Regression for Feature Selection}




I noticed that for 84 movies the ratings are missing. So, I removed the unrated movies, and repeated the analysis for the remaining 1,809 movies, which have 59,918 (binary) features, and are assigned a rating on a scale of 1 to 10. 

In Tables~\ref{tab:lasso} and \ref{tab:lassoCoeff}, I report some statistics of lasso and linear regression for different subsets of the dataset. For example, the first dataset, ``>= 2 occur. singletons'', contains all the features (14,028) that appear in at least two movies. For each dataset, for lasso regression, I report the:
\begin{itemize*}
\item number of features: the number of features included in the corresponding dataset. As a reminder the total number of features is 59,918.
\item lambda: ($\lambda_{minMSE}$) the value of $\lambda$ that corresponds to the minimum MSE.
\item min MSE: the average MSE across the 5-folds for $\lambda_{minMSE}$.
\item SE: the standard deviation of MSE across the 5-folds for $\lambda_{minMSE}$.
\item non-zero coeff.: the total number of non-zero coefficients for $\lambda_{minMSE}$ when {\it all} the data is used. 
\item $\%$ sparsity: percent of zero coefficients in the predictive model.
\item Coeff.~singletons/pairs/triplets: number of non-zero coefficients for each feature type.
\item Top-30 singletons/pairs/triplets: the number of features by type \textit{corresponding to} the top-30 coefficients.
\end{itemize*}
For linear regression, I report:
\begin{itemize*}
\item min MSE: the minimum MSE across the 5-folds
\item mean MSE: the average MSE across the 5-folds 
\item std MSE: the standard deviation MSE across the 5-folds
\item non-zero coeff.: the total number of non-zero coefficients
\end{itemize*}


\begin{observation}
When we include the frequent pairs of features in the dataset (3rd line in Table~\ref{tab:lasso}), the minimum MSE becomes slightly smaller than when we consider only the frequent single features (1.04 vs.~ 1.03). However, the model does pick pairs of features, and slightly smaller number of features compared to the model for the dataset with only frequent singletons.
\end{observation}

==> 040timeModel.tex <==

In this section, we propose a model that can be used when information about the user movie tastes is not available. We assume that all the users will watch the movie eventually, and the time when they watch it follows the exponential distribution Exp$(\lambda_i)$. Under this model, the user conversion function, $f(t)$, which represents the expected number of users that are converted --i.e., watch the movie before time $\tau$-- is given by:
$$f(t) = \sum_{i \in \userSet}P[t_i < \thres] $$

\textbf{Learning.} First we find the weights that maximize the likelihood of the data. Let $\lambda_{ik} = w_i^T f_k$,  the time that user $i$ watches movie $k$ follow the exponential distribution, $y_{ik} \sim \lambda_{ik} exp(-\lambda_{ik} t)$, and $T$ be the time threshold to consider a user converted. Then, we want to maximize the likelihood of the data, or equivalently minimize the negative log-likelihood:
\begin{equation*}
\begin{aligned}
 \text{min} & -logP(D;\lambda) = \\
 & =-log \prod_{i,k,t_{ik}\leq T} \lambda_{ik} exp(-\lambda_{ik} t_{ik}) \prod_{i,k,t_ik > T} exp(-\lambda_{ik} T)\\
 & = - \sum_{i,k,t_{ik}\leq T}(log\lambda_{ik}+\lambda_{ik} t_{ik}) - \sum_{i,k,t_{ik}\geq T} \lambda_{ik} T \Rightarrow \\
 \underset{w_i}{\text{max}} & \sum_{i,k,t_{ik}\leq T}(log\lambda_{ik}+\lambda_{ik} t_{ik}) + \sum_{i,k,t_{ik}\geq T} \lambda_{ik} T \\
 & \text{subject to} \; \; w_i^T f_k > 0 \Rightarrow w_i > 0
 \end{aligned}
 \end{equation*}
 
 This function is a sum of concave functions, and thus is concave itself. Therefore, we can easily find the weights that maximize it.
 
 
 \textbf{User Conversion.} Next, we want to maximize the expected number of users that will get converted. We assume that a user is converted if they are likely to see the movie within $T=20$ days from its release date.
 \begin{equation*}
 \begin{aligned}
& \underset{f_k}{\text{maximize}} 
& & f(\selectedSet)  = \sum_{i \in \userSet}P[t_i < \thres]  \\
& \text{subject to}
& & \sum_{k \in \selectedSet}f_k \leq p, \;\;\;\;\;\;\;\; \text{(Cardinality Constraint)}\\
&&& \sum_{k \in \selectedSet}c_k \dot f_k \leq B, \;\;\;\; \text{(Budget Constraint)} \\
&&& f_k \in \{0,1\}. 
 \end{aligned}
 \end{equation*}
 
 This conversion function is submodular, and thus the we can use the greedy algorithm, which gives a $1-\frac{1}{\epsilon}$ approximation. To convert the decimal solution to integral, we can use pipage rounding \cite{AgeevS04}.
 
 \begin{proof}[Submodularity]
 \reminder{Add the proof of submodularity using the super-negativity argument.}
 \end{proof}
